An FPGA-Based Accelerator Enabling Efficient Support for CNNs with Arbitrary Kernel Sizes

Convolutional neural networks (CNNs) with large kernels, drawing inspiration from the key operations of vision transformers (ViTs), have demonstrated impressive performance in various vision-based applications. To address the issue of computational efficiency degradation in existing designs for supporting large-kernel convolutions, an FPGA-based inference accelerator is proposed for the efficient deployment of CNNs with arbitrary kernel sizes. Firstly, a Z-flow method is presented to optimize the computing data flow by maximizing data reuse opportunity. Besides, the proposed design, incorporating the kernel-segmentation (Kseg) scheme, enables extended support for large-kernel convolutions, significantly reducing the storage requirements for overlapped data. Moreover, based on the analysis of typical block structures in emerging CNNs, vertical-fused (VF) and horizontal-fused (HF) methods are developed to optimize CNN deployments from both computation and transmission perspectives. The proposed hardware accelerator, evaluated on Intel Arria 10 FPGA, achieves up to 3.91 times better DSP efficiency than prior art on the same network. Particularly, it demonstrates efficient support for large-kernel CNNs, achieving throughputs of 169.68 GOPS and 244.55 GOPS for RepLKNet-31 and PyConvResNet-50, respectively, both of which are implemented on hardware for the first time.

==> Background.tex <==
%\vspace{-0.1in}
\section{Background}
%\vspace{-0.1in}
%\subsection{\color{red}{Design Variables And Convolution Operations}}
%\subsection{Detailed Descriptions of Convolution Operations}

%\begin{figure}[hbt]
%\vspace{-1em}
%  \centering
%  \includegraphics[width=7.50cm]{Fig/Fig1.2.pdf}
%  \vspace{-0.1in}
%  \caption{Convolution loop dimensions and design variables.% of loop unrolling and loop tiling.
%  }\label{Fig1}
%\vspace{-0.08in}
%\end{figure}

%The main operation in CNNs is illustrated in Fig.~\ref{Fig1} (a), which involves accumulating the products of input pixels with weights along different dimensions of the kernel and feature maps.
The main operation in CNNs is illustrated in Fig.~\ref{Fig1} (a), where the description dimensions involved in the following sections can be divided into three categories.
Firstly, the sizes of the feature and kernel maps are denoted by convolution loop dimensions ($N*$).
%Due to the decoupling of dependencies across different input channels, i.e., $Nki$ =1, the number of input feature maps ($Nif$) is equal to that of output feature maps ($Nof$).
%In pointwise convolution (PWCV), a $1\times1$ kernel is used to perform independent convolutions on each element of the input feature maps.
Secondly, the sizes of buffered data are determined by loop tiling variables ($T*$), which also affect the latency of DRAM accesses.
An entire row of input pixels and all the input channels in feature maps are buffered in our design, i.e. $Tix=Nix$, $Tif=Nif$, to generate results for a complete row.
Thirdly, the parallel computations are directed by loop unrolling variables ($P*$), where 
$Pox, Poy$, and $Pof$ are set as $8, 8, 16$ in this work.
%\subsection{Typical LKCV-Block Structures}

%\begin{figure}[b]%[hbt]
%\vspace{-1em}
%  \centering
%  \includegraphics[width=8.00cm]{Fig/Fig2.pdf}
%  \vspace{-0.1in}
%  \caption{The architecture of different LKCV blocks.
%  }\label{Fig2}
%\vspace{-0.08in}
%\end{figure}

%For large-kernel CNNs, the typical LKCV-based structures have two main categories: blocks with bypass branches, such as the MBconv and RepLK blocks, and blocks with multiple parallel branches, such as the pyramidal convolution (PyConv) block.
%Specifically, the MBconv block, shown in Fig.~\ref{Fig2} (a), is a commonly used fundamental building block in many lightweight and NAS-based networks.
%The RepLK block is proposed in \cite{RepLKNet2022} to verify the effectiveness of large-kernel design, where each large DWCV uses a $5\times5$ kernel for re-parameterization, as depicted in Fig.~\ref{Fig2} (b).
%Both of these blocks use large-kernel DWCV operations to replace computationally expensive LKCV operations.
%The PyConv block, shown in Fig.~\ref{Fig2} (c), utilizes multi-scale grouped convolutions (group CONV) to enhance the receptive field and improve the ability to capture different levels of details.
%The numbers of output channels and groups in each group CONV can be adjusted to ensure workload balance among different branches.



